First-Generation Inference Accelerator Deployment at Facebook

In this paper, we provide a deep dive into the deployment of inference accelerators at Facebook. Many of our ML workloads have unique characteristics, such as sparse memory accesses, large model sizes, as well as high compute, memory and network bandwidth requirements. We co-designed a high-performance, energy-efficient inference accelerator platform based on these requirements. We describe the inference accelerator platform ecosystem we developed and deployed at Facebook: both hardware, through Open Compute Platform (OCP), and software framework and tooling, through Pytorch/Caffe2/Glow. A characteristic of this ecosystem from the start is its openness to enable a variety of AI accelerators from different vendors. This platform, with six low-power accelerator cards alongside a single-socket host CPU, allows us to serve models of high complexity that cannot be easily or efficiently run on CPUs. We describe various performance optimizations, at both platform and accelerator level, which enables this platform to serve production traffic at Facebook. We also share deployment challenges, lessons learned during performance optimization, as well as provide guidance for future inference hardware co-design.

==> 08-discussion.tex <==
\section{Discussion}
\label{section:discussion}

\subsection{LPDDR vs GDDR/HBM}

Since achieving high energy efficiency in terms of perf/W is a key goal for us, the accelerator cards in our system are designed to operate under a 13W power envelope. Hence as part of the card co-design, we used a low power LPDDR4 memory in the cards. This is different from GDDR5 used in NVIDIA T4, for example.

\subsection{Composability / Flexibility}

\subsection{Sparsity Support}

The NNPI cards have support to store the network weights in compressed format in LLC if the weights are sparse  (i.e. some of the entries in the weight matrix are zero). Hence, one avenue to improve FC performance that we have just started to evaluate is to train the model for having sparse weights. This doesn't affect the computation on NNPI directly (as in, NNPI does not do optimizations to skip over zeros computationally), but we do anticipate significant alleviation of LLC BW pressure that should yield improved performance. Of course, this could result in an accuracy drop as well which needs investigation.

==> 09-lessons_learnt.tex <==
\section{Lessons Learnt}
\label{section:lessons}

We summarize the key lessons learnt as we performed our perf optimizations below. These should be useful when we go to Gen2 or later accelerators.

\vspace{1mm}
\noindent\textbf{Early sharing of micro-benchmarks}: While we had a set of benchmarks we had sent to the vendors prior to chip design, those were not highly targeted and specific to our workloads at hand. Consequently we ended up with a sub-optimal initial starting point with the accelerator. We have now established a set of targeted micro-benchmarks for the vendor which are configurable to be able to reproduce performance on key portions of our workloads of interest. These include individual ops like FC (Gemm), SLS, and Convolutions, as well as system level micro-benches such as PCIe BW in both ideal as well as more realistic traffic conditions. 

\vspace{1mm}
\noindent\textbf{Sharing end-to-end nets}: We set up a methodology for sharing end-to-end nets while not sharing our full SW stack with the vendor. These serialized end-to-end nets are called \textit{Repros}. Sharing end-to-end nets has proven to be immensely helpful in focusing the vendor on the right problems to solve and has been key to our performance improvements.

\vspace{1mm}
\noindent\textbf{Keeping vendors up-to-date with evolving requirements}: Our models evolve over time, and we saw significant changes to the complexity and structure of the models as we went through our performance optimizations. Consequently, performance bottlenecks shifted considerably over time. The end-to-end net sharing mechanism allowed us a concrete way of keeping the vendor up-to-date with the model evolutions on our side, and allowed for appropriate and real-time performance improvements.

\vspace{1mm}
\noindent\textbf{Tooling support for perf evaluations}: First, we had very little initial tooling for finding the high-level system performance bottleneck (host CPU vs NIC vs card). We came up with a way to enable/disable portions of the system for better analysis. Two important examples of this are (a) a way to remove the accelerator performance from the equation using a null kernel that basically returns without executing anything on the accelerator (b) the repro framework for focusing just on the card and PCIe without considering the host CPU. These have turned out to be immensely important tools for perf analysis.

Second, we did not get a stable toolchain from the vendor for finding the trace of operators running on the card for a very long time, giving us very little visibility into what was happening on the card. After receiving this, it immediately gave us a jump in our understanding of performance and opportunities for optimization.

Finally, we lacked a methodology for finding PCIe bottlenecks. It was only when we developed SLS micro-benchmarks and started comparing performance of that to our real model runs did we discover potential PCIe issues and techniques to solve them.

\vspace{1mm}
\noindent\textbf{Facilitating model co-design with high level model characterization tool}: As new model techniques were proposed and standardized over time, our target model also changed significantly. The iterative process of profiling the new model with an actual system, identifying the changes in the bottlenecks, re-prioritizing optimization targets, and communicating with the vendor consumed significant engineering bandwidth. High level performance modeling was very useful in detecting and debugging certain changes and anomalies (e.g., operators assigned to incorrect nets) quickly, as it finishes fast (e.g., within an hour) compared to publishing a model and profiling on a real system which can easily take a day or two. However, the characterization tool itself became unstable from time to time due to the fast-changing landscape of model-related techniques. We expect 1) more frequently synchronizing with model developers to cope with new techniques and maintain the tool’s robustness, and 2) improving the usability of the characterization tool to help model developers to examine the model complexity themselves, would significantly reduce the costs of embracing a new model and help us stay focused on clear performance optimization goals. 




